Evaluating Multi-Instance DNN Inferencing on Multiple Accelerators of an Edge Device

Edge devices like Nvidia Jetson platforms now offer several on-board accelerators -- including GPU CUDA cores, Tensor Cores, and Deep Learning Accelerators (DLA) -- which can be concurrently exploited to boost deep neural network (DNN) inferencing. In this paper, we extend previous work by evaluating the performance impacts of running multiple instances of the ResNet50 model concurrently across these heterogeneous components. We detail the effects of varying batch sizes and hardware combinations on throughput and latency. Our expanded analysis highlights not only the benefits of combining CUDA and Tensor Cores, but also the performance degradation from resource contention when integrating DLAs. These findings, together with insights on precision constraints and workload allocation challenges, motivate further exploration of intelligent scheduling mechanisms to optimize resource utilization on edge platforms.

==> usepackages.tex <==
%,onecolumn,12pt
%\documentclass{IEEEtran}
% Some/most Computer Society conferences require the compsoc mode option,
% but others may want the standard conference format.
%
% If IEEEtran.cls has not been installed into the LaTeX system files,
% manually specify the path to it like:
% \documentclass[conference,compsoc]{../sty/IEEEtran}

% \IEEEoverridecommandlockouts
% % The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Additional fonts
\usepackage[T1]{fontenc} %% https://tex.stackexchange.com/questions/664/why-should-i-use-usepackaget1fontenc
%\usepackage{lmodern} %% https://tex.stackexchange.com/questions/2369/why-do-the-less-than-symbol-and-the-greater-than-symbol-appear-wrong-as
\usepackage[normalem]{ulem} % required for strikeout font
% Default Computer Modern font (no bold implemented)
%\renewcommand{\ttdefault}{cmtt}
% Hence, Using Courier font
\renewcommand{\ttdefault}{pcr}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Inline comments. Pick initials and color of your choice. \ysnote{} refers to Yogesh's note. 
%
\usepackage[usenames,dvipsnames,svgnames,x11names]{xcolor}
\newcommand{\nbc}[3]{
 {\colorbox{#3}{\bfseries\sffamily\scriptsize\textcolor{white}{#1}}}
 {\textcolor{#3}{\sf\small$\blacktriangleright$\textit{#2}~$\blacktriangleleft$}}
}

\newcommand{\ysnote}[1]{\nbc{YS}{#1}{magenta}}
\newcommand{\drnote}[1]{\nbc{DR}{#1}{orange}}
\newcommand{\ysnoted}[1]{\nbc{LATER}{#1}{green}} % postpone addressing of comment

% \newcommand{\ysnote}[1]{ {\textcolor{magenta} { ***Yogesh: #1 }}} % needs a response
% \newcommand{\drnote}[1]{ {\textcolor{orange} { ***Dreamer: #1 }}}
\newcommand{\Note}[1]{\textcolor{red}{#1}} % verify if this is correct


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Change tracking for article revisions. Added, Deleted, Replaced, or Modified content.
%
\newcommand{\modc}[1]{{\textcolor{blue}{#1}}}
\newcommand{\addc}[1]{{\textcolor{teal}{#1}}}
%% NOTE: \sout will break if the text has citations with an error that there is an extra "}". Place the citation within mbox: \mbox{foo~\cite{foo}}
\newcommand{\delc}[1]{ {\textcolor{gray} {\sout{#1}} }}
%\newcommand{\delc}[1]{} % uncomment this (and comment above line) to ignore showing deletion
\newcommand{\repc}[2]{ {\textcolor{gray} {\sout{#1}} }{\textcolor{teal} {#2}}}
%\newcommand{\repc}[2]{{\textcolor{teal}{#2}}} % uncomment this (and comment above line) to ignore showing deletion
%
%---------------------------------------------------------


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%
%%% UNCOMMENT THE SECTION BELOW TO REMOVE CHANGE TRACKING/COMMENTS
%%%%%%
% \renewcommand{\ysnote}[1]{} % remove comment text
% \renewcommand{\drnote}[1]{} % remove comment text
% \renewcommand{\Note}[1]{#1} % remove red font color, retain text
% \renewcommand{\ysnoted}[1]{} % remove comment text
% \renewcommand{\srnote}[1]{} % remove comment text
% \renewcommand{\rrnote}[1]{} % remove comment text
% \renewcommand{\rrnoted}[1]{} % remove comment text
% \renewcommand{\hgnote}[1]{} % remove comment text
% \renewcommand{\modc}[1]{#1} % remove font color, retain text
% \renewcommand{\addc}[1]{#1} % remove font color, retain text
% \renewcommand{\delc}[1]{} % remove deleted text
% \renewcommand{\repc}[2]{#2} % remove deleted text, remove font color and retain added text

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% *** MISC UTILITY PACKAGES ***
%
%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%   % dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/pkg/ifpdf
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% *** CITATION PACKAGES ***
%
\usepackage[nocompress]{cite}
% cite.sty was written by Donald Arseneau
% V1.6 and later of IEEEtran pre-defines the format of the cite.sty package
% \cite{} output to follow that of the IEEE. Loading the cite package will
% result in citation numbers being automatically sorted and properly
% "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% \cite will automatically add leading space, if needed. Use cite.sty's
% noadjust option (cite.sty V3.8 and later) if you want to turn this off
% such as if a citation ever needs to be enclosed in parenthesis.
% cite.sty is already installed on most LaTeX systems. Be sure and use
% version 5.0 (2009-03-20) and later if using hyperref.sty.
% The latest version can be obtained at:
% http://www.ctan.org/pkg/cite
% The documentation is contained in the cite.sty file itself.
%
% Note that some packages require special options to format as the Computer
% Society requires. In particular, Computer Society  papers do not use
% compressed citation ranges as is done in typical IEEE papers
% (e.g., [1]-[4]). Instead, they list every citation separately in order
% (e.g., [1], [2], [3], [4]). To get the latter we need to load the cite
% package with the nocompress option which is supported by cite.sty v4.0
% and later.

%% Balances the bibliography columns in last page
\usepackage{balance}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% When using XML fragments, using pretty-print is helpful.
%
\usepackage{listings}
% \usepackage{color}
% \definecolor{gray}{rgb}{0.4,0.4,0.4}
% \definecolor{darkblue}{rgb}{0.0,0.0,0.6}
%\definecolor{maroon}{rgb}{0.5,0,0}
% \definecolor{cyan}{rgb}{0.0,0.6,0.6}

\lstset{
  basicstyle=\ttfamily,
  columns=fullflexible,
  breaklines=true,
  showstringspaces=false,
  commentstyle=\color{gray}\upshape,
  escapeinside={||},
  mathescape=true
}

\lstdefinelanguage{XML}
{
basicstyle=\ttfamily\footnotesize,
  morestring=[b]",
  moredelim=[s][\bfseries\color{Maroon}]{<}{\ },
  moredelim=[s][\bfseries\color{Maroon}]{</}{>},
  moredelim=[l][\bfseries\color{Maroon}]{/>},
  moredelim=[l][\bfseries\color{Maroon}]{>},
  morecomment=[s]{<?}{?>},
  morecomment=[s]{<!--}{-->},
  commentstyle=\color{gray},
  stringstyle=\color{blue},
  identifierstyle=\color{red}
%  morekeywords={type,id,value,impl}% list your attributes here
}
%
%---------------------------------------------------------


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Better control over verbatim text
\usepackage{moreverb}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% for syntax/grammar
\usepackage[nounderscore]{syntax}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[pdftex]{graphicx}
% declare the path(s) where your graphic files are
\graphicspath{{./figures/}}
% and their extensions so you won't have to specify these with
% every instance of \includegraphics
\DeclareGraphicsExtensions{.pdf}
% graphicx was written by David Carlisle and Sebastian Rahtz. It is
% required if you want graphics, photos, etc. graphicx.sty is already
% installed on most LaTeX systems. The latest version and documentation
% can be obtained at: 
% http://www.ctan.org/pkg/graphicx
% Another good source of documentation is "Using Imported Graphics in
% LaTeX2e" by Keith Reckdahl which can be found at:
% http://www.ctan.org/pkg/epslatex
%
% latex, and pdflatex in dvi mode, support graphics in encapsulated
% postscript (.eps) format. pdflatex in pdf mode supports graphics
% in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure
% that all non-photo figures use a vector format (.eps, .pdf, .mps) and
% not a bitmapped formats (.jpeg, .png). The IEEE frowns on bitmapped formats
% which can result in "jaggedy"/blurry rendering of lines and letters as
% well as large increases in file sizes.
%
% You can find documentation about the pdfTeX application at:
% http://www.tug.org/applications/pdftex

% Definitions for placeholder figures
\newcommand{\dummyfigX}{\fbox{\parbox[h][1.75in][t]{0.95\textwidth}{\emph{Placeholder}}}} % full page width (figure*)
\newcommand{\dummyfigXX}{\fbox{\parbox[h][1.75in][t]{0.95\columnwidth}{\emph{Placeholder}}}} % 1 column width (in 2 column format)
\newcommand{\dummyfigXXX}{\fbox{\parbox[h][1.75in][t]{0.30\textwidth}{\emph{Placeholder}}}} % 1/3 full page width (figure*)
\newcommand{\dummyfigXXXX}{\fbox{\parbox[h][1.75in][t]{0.23\textwidth}{\emph{Placeholder}}}} % 1/4 full page width (figure*)


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% *** MATH PACKAGES ***
%
\usepackage[cmex10]{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{amsfonts}
% \usepackage{gensymb}

\newtheorem{cons}{Constraint}
%
% A popular package from the American Mathematical Society that provides
% many useful and powerful commands for dealing with mathematics.
%
% Note that the amsmath package sets \interdisplaylinepenalty to 10000
% thus preventing page breaks from occurring within multiline equations. Use:
%\interdisplaylinepenalty=2500
% after loading amsmath to restore such page breaks as IEEEtran.cls normally
% does. amsmath.sty is already installed on most LaTeX systems. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/amsmath



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% *** SUBFIGURE PACKAGES ***
\usepackage{subfig} %[caption=false,font=footnotesize,labelfont=sf,textfont=sf]
%
% subfig.sty, written by Steven Douglas Cochran, is the modern replacement
% for subfigure.sty, the latter of which is no longer maintained and is
% incompatible with some LaTeX packages including fixltx2e. However,
% subfig.sty requires and automatically loads Axel Sommerfeldt's caption.sty
% which will override IEEEtran.cls' handling of captions and this will result
% in non-IEEE style figure/table captions. To prevent this problem, be sure
% and invoke subfig.sty's "caption=false" package option (available since
% subfig.sty version 1.3, 2005/06/28) as this is will preserve IEEEtran.cls
% handling of captions.
% Note that the Computer Society format requires a sans serif font rather
% than the serif font used in traditional IEEE formatting and thus the need
% to invoke different subfig.sty package options depending on whether
% compsoc mode has been enabled.
%
% The latest version and documentation of subfig.sty can be obtained at:
% http://www.ctan.org/pkg/subfig




% *** SPECIALIZED LIST PACKAGES ***
%
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage[ruled]{algorithm}
\definecolor{light-gray}{gray}{0.75}
\algrenewcommand{\algorithmiccomment}[1]{\hskip3em{{\footnotesize \textcolor{light-gray}{$\blacktriangleright$}}} #1}
%
% This package provides an algorithmic environment fo describing algorithms.
% You can use the algorithmic environment in-text or within a figure
% environment to provide for a floating algorithm. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Table relates packages
\usepackage{multirow} % Multi-row tables
\usepackage{rotating} % sideways table
\usepackage{booktabs} % better lines
\usepackage{colortbl} % cell colors
\usepackage{tablefootnote} % add support for footnote in table

\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% *** PDF, URL AND HYPERLINK PACKAGES ***
%
%\usepackage[colorlinks,bookmarksopen,bookmarksnumbered,citecolor=red,urlcolor=red,pagebackref=true]{hyperref}
\usepackage[pdftex,colorlinks=true,urlcolor=blue,citecolor=blue]{hyperref}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Avoids contiguous empty spaces
\usepackage{xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% IEEETrans class fix for enumitem. provide for legacy IED commands/lengths when possible
% http://comments.gmane.org/gmane.editors.lyx.general/68611
\let\labelindent\relax
\usepackage{enumitem}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% correct bad hyphenation here
\hyphenation{compu-ta-tio-nal}

% define repetitive complex fragments here
\newcommand{\floe}{$\mathcal{F}{\ell}{o}{\varepsilon}$\xspace}
\newcommand{\prc}{\mathcal{P}}
\newcommand{\chn}{\mathcal{C}}
\usepackage{caption}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% generate lorum ipsum placeholder text
%\usepackage[english]{babel}
\usepackage{blindtext}
\newcommand{\blindtextc}{\color{gray}\blindtext\color{black}}
\newcommand{\Blindtextc}{\color{gray}\Blindtext\color{black}}


